Attribute or Abstain: Large Language Models as Long Document Assistants

LLMs can help humans working with long documents, but are known to hallucinate. Attribution can increase trust in LLM responses: The LLM provides evidence that supports its response, which enhances verifiability. Existing approaches to attribution have only been evaluated in RAG settings, where the initial retrieval confounds LLM performance. This is crucially different from the long document setting, where retrieval is not needed, but could help. Thus, a long document specific evaluation of attribution is missing. To fill this gap, we present LAB, a benchmark of 6 diverse long document tasks with attribution, and experiments with different approaches to attribution on 5 LLMs of different sizes. We find that citation, i.e. response generation and evidence extraction in one step, performs best for large and fine-tuned models, while additional retrieval can help for small, prompted models. We investigate whether the "Lost in the Middle'' phenomenon exists for attribution, but do not find this. We also find that evidence quality can predict response quality on datasets with simple responses, but not so for complex responses, as models struggle with providing evidence for complex claims.

==> tex/formalization.tex <==

\begin{figure*}
    \centering
    \includegraphics{img/Attribution_detailed.drawio.pdf}
    \caption{The approaches to attribution tested in this work. For details, see §\ref{sec:formalization/approaches}.}
    \label{fig:attribution}
\end{figure*}

\paragraph{Task definition} 
\label{sec:formalization/task_definition}
We assume an instruction $I$ (a general task description and optionally instance-specific input, e.g. a question or a claim) and a context document $D$ consisting of a set of segments ${d}$ (typically paragraphs). The expected output consists of a task specific response $R$ (e.g. an answer to a question or an entailment label), consisting of one or multiple statements $\{r\}$, and an evidence set $\mathcal{E}=\{E\}$. Each $E_i$ contains evidence segments: $E_i \subset D$. Statement $r_i$, should be \textit{attributable} to $E_i$. \\
Note that there are responses that do not need evidence, (e.g. ``unanswerable'' in question answering or ``not supported'' in fact checking).

\paragraph{Approaches}
\label{sec:formalization/approaches}
 These can be solved simultaneously or sequentially, resulting in three approaches to attribution defined in §\ref{sec:introduction}: (1) \texttt{post-hoc}, (2) \texttt{retrieve-then-read} and (3) \texttt{citation} \cite{bohnet2022attributed, gao2023alce, malaviya2024expertqa}. Several works have reduced long inputs to the most salient passages before using them as input to LLMs \cite{xu2024retrieval, bai2023longbench}, some finding a positive effect on performance. We follow these works to get additional approaches (4) \texttt{reduced-post-hoc} and (5) \texttt{reduced-citation}. In each of these, an initial retrieval step is performed on the input document to get $D' \subset D$, which is used as input instead of $D$ \footnote{Following other works \cite{bohnet2022attributed, gao2023alce, malaviya2024expertqa}, evidence retrieval in \texttt{post-hoc} is performed on the complete document $D$.}. See Fig.~\ref{fig:attribution} for a visualization.


==> tex/tmp_rel_work.tex <==
\paragraph{Attribution}
Contrast to Explainability we do not care about the internal decision process of the model, but rather trustworthiness of the answer. Similar to a post hoc explanation.

%Short background and gap
The concept of "attributability" was introduced by Rashkin et al. [cite], where a statement \textit{s} is attributable to an information source \textit{P} if “According to \textit{P}, \textit{s}” holds. They give a formal treatment of the problem and study the human evaluation of attributability. Attribution, the task of selecting the parts of the model input to which the output is attributable, has mostly been studied in two settings: short input texts [cite] and retrieve-and-read scenarios [cite]. 
\begin{itemize}
    \item \textbf{Evaluation}
    \item Rashkin et al
    \item Automatic evaluation of attribution by LLMs (Yue 2023): Create 2 datasets for automatic evaluation of attribution, find that GPT-4 works best.
    \item Evaluating Verifiability in Generative Search Engines (Liu et al, 2023): Human eval of several commercial generative search engines as to whether the generated statements are supported by the given citations and the proportion of citations that are relevant.
    \item Benchmarking LLMs in Complex QA attribution using KGs (Hu 2024): Create a dataset to evaluate Attribution evaluation models from KGs. Find that fine-tuned models work much better. 
    \item \textbf{Retrieve-then-read scenarios}
    \item Gophercite (Menick et al, 2022): Given a question, web retrieval returns relevant passages. Gopher 280B is fine tuned via RLHF to answer the question and quote the evidence. Model gets the option t decline to answer.
    \item WebGPT
    \item Enabling LLMs to Generate Text with Citations (ALCE) - Gao et al 2023: Test several LLMs in a retrieve then read scenario  with long form QA, each sentence is to be cited, few retrieved passages for OS models, but ChatGPT and GPT-4 evaluated with up to 20 passages.
    \item Attributed Question Answering (Bohnet et al, 2023): Try to get attributed answers to NQ in full wiki setting. They experiment with retrieve then read, post hoc retrieval and LLM as retriever via generation of URL.
    \item Evaluating and modeling attribution for Cross Lingual QA (Muller et al, 2023): They use an existing model for open book retrieve then read multilingual QA and evaluate the attributability of answers, which is surprisingly low. They evaluate several models for automatic evaluation of attributability and use these models to improve attributability.
    \item Llatrieval: Use an LLM to select best retrieval results or even make additional queries, evaluated on ALCE
    \item RARR (Gao et al, 2023): Texts are revised according to evidence retrieved from web search, but LLMs do not retrieve evidence. 
    \item HAGRID (Kamalloo, 2023): Dataset of questions, text snippets and answers, in which each sentence has to reference at least one text snippet. GPT 3.5 generates attributes answers and humans validate. Only ~3 snippets per question. No model evaluation
    \item Training Language Models to Generate Texts with Citations... Huang 2024: Training method to make LLMs cite relevant parts of input, evaluated on ALCE and ExpertQA
    \item \textbf{Other}
    \item Make your decision convincing! (Du et al, 2023): Use finetuned models (LongT5 and BERT) to first extract rationale and then predict question based on rationale. Evaluate on 5 ERASER datasets
    \item Evidentiality guided generation for knowleddge intensive NLP tasks (Asai et al, 2022): Train an FiD model multi task to predict evidence and answer, evidence prediction is supervised with silver labels.
    \item Grounding Language Model with Chunking-Free... (Qian et al, 2024): They train a model to generate evidence from long docs via constrained decoding.
    \item Towards faithful and robust LLM specialists for evidence-based QA (Schimanski 2024): Create train and several test datasets to train and evaluate models to create attributed answers. Between 5 and 10 paragraphs / instance.
    \item SAIL (Luo, 2023): They fine-tune a small model to first evaluate usefulness of search results before generating an answer.
\end{itemize}

Gap: No evaluation in long document scenarios.

\paragraph{Answerability}
\begin{itemize}
    \item Towards reliable and factual response generation (Lajewska 2024): Create a dataset of questions and relevant / irrelevant passages, train a sentence level model to predict if a sentence contains relevant info
    \item NoMIRACL (Thakur, 2024): Models get relevant / irrelevant passages and need to decide if question is answerable
    \item Know what you don't know (Squad 2.0, Rajpurkar 2018): Add unanswerable questions to Squad
    \item Challenges in information seeking QA (Asai 2021): Investigation of unanswerability in NQ and TydiQA: Performance when given gold long answer / question type, prediction of unanswerability, analysis of unanswerable questions
    \item Does it Know (Huang 2023): Train a classifier to predict yes / no / unanswerable without explicit supervision
    \item LMs mostly know what they know (kadavath 2023): LMs are well-calibrated on multiple choice, models trained to predict answerability (without context) are well-calibrated.
    \item Yes, No or IDK (Sulem, 2022): Add unanswerable questions to BoolQ, training on MNLI helps to solve the new dataset. 
    \item PTAU (Liao 2022): Train a special model (BERT or RoBERTa based) to predict causes of unanswerability on Squad2-CR
    \item Knowledge of Knowledge (Amayuelas 2023): Create a dataset with questions whose answer is unknown and test performance of LLMs to identify these questions
    \item The curious case of hallucinatory unanswerability (Slobodkin 2023): Test whether models can predict unanswerability in QA with short context and train linear layers to do the prediction
    \item Cognitive Dissonance (Liu 2023): They investigate the match / mismatch between predictions from probes and queries (token outputs). 
\end{itemize}

Gap: No research in long document scenarios

\paragraph{Long Context LLMs}
\begin{itemize}
    \item LongAlign (Bai 2024): Instruction tuning data, eval data and training strategy for long doc LLMs. Their related work categorizes Long LLM approaches into with fine tuning and without fine-tuning. 
    \begin{itemize}
        \item With fine-tuning: Position encoding extension and continual pretraining data on longer sequences. E.g. Chen et al 2023 positional interpolation, Peng 2023 Yarn, Xiong 2023 effective long context scaling (Meta, models not public), Chen 2023 LongLora, 
        \item Without fine-tuning: Sliding window attention: Han 2023 Lm-infinite. Token compression: Jiang 2023 prompt compression, Jiang 2024 activation beacon
    \end{itemize}
    \item \textbf{Other context extension approaches}
    \item GritLM: Can do both embedding and generation, based on Mistral
    \item Parallel context window (Ratner 2023): Similar to FiD but with LLMs
    \item Focused Transformer (Tworkowski 2023): Some transformer layers can attent to vector memory via kNN search
    \item Landmark attention (2023): Context divided into blocks, each block receives special token
    \item \textbf{Improving use of context}
    \item Retrieval meets LLMs (Xu 2023): Top 5 retrieval improves short- and long context LLMs on Long Doc tasks.
    \item RAPTOR (Sarthi 2024): Chunk long document, then cluster and summarize, then repeat. Then retrieve from the tree and use as input to reader.
    \item PEARL (Sun 2023): LLM first generates plan of actions on long doc, which is then executed one by one to get final answer. 
    \item Walking down the memory maze (Chen 2023): Similar to RAPTOR / Drilling down into the discourse structure
    \item \textbf{Analysis of context usage}
    \item Lost in the Middle: Multi doc QA performance deteriorates when relevant context is in the middle. Similar for synthetic retrieval task. Putting instruction before and after context can help. 
    \item On context utilization in summarization with large language models: Model summaries exhibit more similarity to beginning / end of articles, models struggle when relevant documents are in the middle in multi doc summarization.
\end{itemize}

\paragraph{Reranking / extraction with LLMs}
\begin{itemize}
    \item Reranking
    \begin{itemize}
        \item Several approaches to use LLMs to rerank retrieval results: Is ChatGPT good at search (Sun 2023), RankVicuna (Pradeep 2023), RankZephyr (Pradeep 2023): Listwise reranking works well. 
        \item Attention sorting (Peysakhovich 2023): Use attention values to sort passages in context iteratively.
        \item LLMs for retrieval survey (Zhu 2023): GPT 4 can do listwise reranking well, smaller models are worse
        \item LLMs are effective text rankers with pairwise ranking prompting (2023)
        
    \end{itemize}
    \item Drilling down into discourse structure (Nair 2023): First summarize sections and input summaries to ChatGPT, it selects sections and then retrieves from these. 
    \item PDFTriage (Saad-Falcon 2023): Augmented ChatGPT with functions to retrieve document content, it gets only document metadata and then needs to use the functions. Evaluated on new dataset. 
    \item WebGPT (Nakano 2022): LLM is trained to cite relevand passages. 
    \item Never lost in the Middle (He 2023): Model is trained to first repeat question, then generate doc indices and then generate answer. No eval on long docs
    \item Honest students from untrusted teachers (Eisenstein 2022): Models need to quote evidence from decontextualized paragraphs
\end{itemize}

Gap: No research in full long document scenarios. No evaluation of embedding-based approaches. 

\paragraph{Further dataset candidates}
\begin{itemize}
    \item QASA: Paber based QA with more challenging questions than QASPER, each evidence paragraph is annotated with rationale
    \item LooGLE
\end{itemize}

\paragraph{Benchmarks}
\begin{itemize}
    \item Marathon: 6 tasks, 60k to 260k+, multiple choice questions. Created based on Loogle and Longbench. Extraction not evaluated
    \item M4LE: 36 datasets, 11 task types, 12 domains, 1k to 8k, they reuse existing (party short context datasets) and combine paragraphs to get long context datasets. Extraction not evaluated
    \item LV-Eval: 16k to 256k tokens. Tasks are single- and multi hop QA. Contexts are synthetic (not single documents). No evidence.
    \item LooGle: 20k words on average. summarization (on arxiv), single and multi context QA (Wikipedia and movie scripts), partly with annotated evidence. Can probably use the QA part.
    \item LongBench: variety of tasks between 1k and 18k length, QA, multi doc QA, passage retrieval, ... . No annotated evidence, but passage retrieval is extraction task
    \item BAMBOO: QA, hallucination detection, passage reordering, text completion and code completion, 3k to 8k, no evidence, passage reordering could be seen as extraction
    \item L-Eval: avg length between 4k to 60k, English, closed-ended (multiple choice QA, topic retrieval, math problems) and open ended (QA, summarization, extracting key information) tasks. No evidence. 
    \item ZeroScrolls: 2k to 50k words, Summarization, QA, aggregation (determine percentage of positive reviews, sorting book chapter summaries), no evidence
    \item KILT: Benchmark of datasets all mapped to the same Wikipedia snapshot. Models are evaluated with the respective dataset metrics and for retrieval of complete wikipedia pages.
    \item ERASER: Benchmark for tasks with extractive explanations. Models are evaluated both for the end task metric and for their rationales (token overlap with human rationales, comprehensiveness and sufficiency). Evidence Inference and BoolQ could be long doc. 
\end{itemize}

Gap: No evaluation of extraction / attribution.

\paragraph{Self-correction}

\begin{itemize}
    \item \todo{Long Documents / Retrieval?}
    \item Adaptation with Self-Evaluation to improve Selective Prediction... (Chen 2023): Rather complex method to train a model to decide when it should not answer
    \item Self-evaluation improves selective generation... (Ren 2023): Sample multiple answers from LLM and let it rate them in a multiple choice fashion (better than using sequence probability).
\end{itemize}
